A Survey on Graph Drawing Beyond Planarity

Graph Drawing Beyond Planarity is a rapidly growing research area that classifies and studies geometric representations of non-planar graphs in terms of forbidden crossing configurations. Aim of this survey is to describe the main research directions in this area, the most prominent known results, and some of the most challenging open problems.

==> beyond.tex <==
 The scientific literature on the treatment of edge crossings in graph visualization embraces other topics that have not been discussed in the previous sections of this survey and that are mentioned here. Although these topics are not usually recognized as part of the literature on graph drawing beyond planarity, they are clearly related and recent works establish interesting contact points with beyond-planar graph families.

%\subsection{Additional Structural Properties} \label{ss:additional}
%
%An exhaustive survey of the results about structural properties of $1$-planar graphs can be found in~\cite{DBLP:journals/csr/KobourovLM17}. Among the most relevant results, we mention that $1$-planar graphs have chromatic number six~\cite{B95} and book thickness at most $39$~\cite{DBLP:journals/algorithmica/BekosBKR17}. 
%
%For $k$-planar graphs on $n$ vertices, it is known that they have $O(\log n)$ book thickness~\cite{JGAA-454}, $O(\sqrt{kn})$ treewidth and $O(k)$ layered treewidth~\cite{DBLP:journals/siamdm/DujmovicEW17}, and bounded expansion~\cite{NesetrilMW12}.
%
%
%\begin{description}
%  \item[stack number] 
%  \item[queue number]
%  \item[partition] 
%  \item[page number] 
%  \item{boh?}
%\end{description}

%\subsection{Other Related Topics}\label{ss:other} 

\myparagraph{Crossing Minimization.} Given a graph $G$, finding a drawing $\Gamma$ of $G$ with the minimum number of edge crossings is one of the oldest and most studied problems in graph drawing, often recognized as the \emph{crossing minimization problem} for $G$; the number of crossings of $\Gamma$ is the \emph{crossing number of $G$}. Restrictions of the definition of crossing number have also been considered; for example, if we require that the drawing of $G$ has straight-line edges, the crossing number of $G$ may be higher than in the general case. Refer to~\cite{schaefer-13} for a survey on the different variants of crossing number studied in the literature. It is well known that the crossing minimization problem is \npc~\cite{gj-79} and it remains hard also in very restricted scenarios, for instance when the graph is bipartite and we look for a straight-line $2$-layer drawing of it~\cite{gj-83}. Polynomial-time heuristics and exponential-time exact algorithms for the crossing minimization problem are described and experimented in the literature, both in the general case and in different constrained settings (see, e.g.,~\cite{DBLP:reference/crc/BuchheimCGJM13} for a survey). Nonetheless, the crossing minimization problem might be polynomial-time solvable for some beyond-planar graph families; for example, this is the case for $2$-layer RAC drawable graphs~\cite{DBLP:journals/algorithmica/GiacomoDEL14}. This observation motivates the study of the crossing minimization problem under forbidden crossing configurations. 

\myparagraph{Relaxed Clustered Planarity.} Clustered planarity is a research topic motivated by several real-world visualization scenarios. In a \emph{clustered graph}, vertices are grouped into clusters, which may be hierarchically organized. 
%As an example, think of a collaborative network in which the vertices represent persons of different countries that cooperate in some activities, and where an edge between two vertices witnesses a cooperation between the corresponding persons. In such a network, persons may be grouped into clusters according to their geographic area; again, the persons in each cluster may be grouped based on some other criterion such as level of expertise or type of skills. 
In a layout of the clustered network each cluster should be clearly represented as a closed region containing all (and only) its vertices and all (and only) its subclusters, in a recursive fashion. Also, an edge should not traverse (i.e., cut) a cluster if both its endvertices are outside the cluster. 
Many papers tackled the problem of testing whether a clustered planar graph admits a crossing-free drawing that meets the aforementioned properties (see the surveys~\cite{kw-dg-01,DBLP:conf/compgeom/CorteseB05}) and practical planarization and drawing heuristics have also been conceived, even for non-planar and large graphs (e.g.,~\cite{DBLP:conf/gd/BattistaDM01,DBLP:conf/iv/BourquiAM07,DBLP:conf/apvis/OmoteS07,DBLP:journals/isci/DogrusozGCCD09,DBLP:journals/isci/DidimoM14}). Recently, a relaxed version of the clustered planarity model has been proposed, in which some types of crossings (between two edges, between two regions, or between an edge and a region) are allowed in a limited measure, and trade-offs between different types of crossings are studied~\cite{DBLP:journals/comgeo/AngeliniLBFPR15}. This extension of the classical clustered planarity setting goes in the same direction as the research in graph drawing beyond planarity. 
   
\myparagraph{Hybrid Visualizations.} In order to diminish the negative effect of visual clutter caused by the presence of many edge crossings in large and locally dense networks, the use of matrix-based representations combined with the classical node-link representation has been explored. A matrix-based representation of a graph $G$ is a visualization of the adjacency matrix of $G$, where the order of the vertices along rows and columns of the matrix can be fixed or freely chosen. Hybrid visualizations that mix node-link and matrix-based representations are proposed for the first time in a system for the visual analysis of social networks, called \textsc{NodeTrix}~\cite{DBLP:journals/tvcg/HenryFM07}. The basic idea is to visualize dense subgraph as matrices, while the rest of the graph is still drawn in a classical node-link style. Hybrid visualizations are also used in combination with graph clustering algorithms that guarantee specific properties in terms of planarity of the inter-cluster graph~\cite{DBLP:journals/tvcg/BatageljBDLPP11}. More recently, the planarity testing and embedding problem of hybrid visualizations in the \textsc{NodeTrix} model has been further formalized and studied, assuming that the input graph is already clustered and that each cluster is represented as a matrix~\cite{DBLP:conf/gd/LozzoBFP16,nodetrix-gd17}.

\myparagraph{Edge Bundling.} The idea of grouping edges to compute planar drawings of non-planar graphs with no loss of information was originally proposed and theoretically studied in the graph drawing community, using the term \emph{confluent drawings}~\cite{DBLP:journals/jgaa/DickersonEGM05,DBLP:journals/algorithmica/EppsteinGM07}. Later on, as for hybrid visualizations, edge-bundling approaches were introduced in the information visualization area to address the visual-clutter problem in node-link diagrams of large dense graphs~\cite{DBLP:journals/tvcg/Holten06}. The basic idea of this second line of research is that ``similar'' edges are deformed and grouped into bundles, thus providing a more abstract and uncluttered view of the original drawing at the expenses of possible ambiguities in terms of connections between specific pairs of vertices.
There are many types of edge-bundling algorithms, using geometric graphs, trees, or parallel coordinates plots; they rely on different approaches, such as force-directed, geometry-based, and image-based approaches (see, e.g., the surveys~\cite{DBLP:journals/cgf/HoltenW09,zxyq-13}. Very recently, the use of edge bundling has been formally studied in the context of graph drawing beyond planarity, with the introduction of a new family of beyond-planar graphs called \emph{1-fan-bundle planar} graphs, which combines edge bundling with fan-planar graphs~\cite{1-fbp-gd17}. The use of fan-planar drawings to support edge bundling was originally suggested in a previous work as a motivation to study this graph family~\cite{DBLP:journals/tcs/BinucciGDMPST15} (see also Figure~\ref{fi:fan-planarity}).   


%\begin{itemize}
%\item Crossing Minimization
%\item Cluster Planarity and Beyond
%\item Exploring large and complex networks
%	\begin{itemize}
%	\item Hybrid visualizations (matrix-based + node-link)
%	\item Techniques for reducing the visual complexity caused by the edges (edge bundling, ..)
%	\item Parallel and Distributed platforms
%	\end{itemize}
%\end{itemize} 
